Lessons Learned Addressing Dataset Bias in Model-Based Candidate Generation at Twitter

Traditionally, heuristic methods are used to generate candidates for large scale recommender systems. Model-based candidate generation promises multiple potential advantages, primarily that we can explicitly optimize the same objective as the downstream ranking model. However, large scale model-based candidate generation approaches suffer from dataset bias problems caused by the infeasibility of obtaining representative data on very irrelevant candidates. Popular techniques to correct dataset bias, such as inverse propensity scoring, do not work well in the context of candidate generation. We first explore the dynamics of the dataset bias problem and then demonstrate how to use random sampling techniques to mitigate it. Finally, in a novel application of fine-tuning, we show performance gains when applying our candidate generation system to Twitter's home timeline.

==> tables/best_cl.tex <==
\begin{table}
  \centering
  \begin{tabular}{|l|l|l|}
    \hline
    & Control & CL Model \\ \hline
    Fav \(\%\) & 3.6 & 4.3 \\ \hline
    Reply \(\%\) & 0.04 & 0.07 \\ \hline
    Retweet \(\%\) & 0.8 & 1.0 \\ \hline
  \end{tabular}
  \caption{Further improvements in CL with ranker and requesting more candidates from ANN.}
  \label{tab:best_cl}
\end{table}


==> tables/ddg9583.tex <==
\begin{table*}[!htb]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
\hline
\multicolumn{1}{c}{Metrics} & Control & \begin{tabular}[c]{@{}c@{}}Base CL model\\ requesting 20 candidates\end{tabular} & \begin{tabular}[c]{@{}c@{}}Base CL model\\ requesting 200 candidates\end{tabular} & \begin{tabular}[c]{@{}c@{}}Using fixed ann score threshold\\ for selection with 20 candidates\end{tabular} & \begin{tabular}[c]{@{}c@{}}Using fixed ann score threshold\\ for selection with 200 candidates\end{tabular} \\ \hline \hline
Fav (\%) & 3.6 & 3.4 & 3.6 & 3.9 & 4.3 \\ \hline
Reply (\%) & 0.04 & 0.05 & 0.07 & 0.05 & 0.07 \\ \hline
Retweet (\%) & 0.8 & 0.7 & 0.8 & 0.8 & 1.0 \\ \hline
\end{tabular}%
}
\caption{DDG 9583}
\label{tab:ddg9583}
\end{table*}

==> tables/pretrain_vs_cl.tex <==
\begin{table}
  \centering
  \begin{tabular}{|l|1|1|1|}
    \hline
    & Control & Yml Pretrain Model & CL Model \\ \hline
    Fav \(\%\) & 2.51 & 1.46 & 3.19 \\ \hline
    Reply \(\%\) & 0.049 & 0.036 & 0.046 \\ \hline
    Retweet \(\%\) & 0.70 & 0.35 & 0.65 \\ \hline
  \end{tabular}
  \caption{}
  \label{tab:pretrain_vs_cl}
\end{table}


==> tables/triplet_ddg_results.tex <==
\begin{table}
  \centering
  \begin{tabular}{|l|l|l|}
    \hline
    & Control & Triplet \\ \hline
    Fav \(\%\) & 3.0 & 2.0 \\ \hline
    Reply \(\%\) & 0.04 & 0.08 \\ \hline
    Retweet \(\%\) & 0.66 & 0.48 \\ \hline
  \end{tabular}
  \caption{}
  \label{tab:triplet_ddg_results}
\end{table}

